Vision-Based Autonomous Drone Control using Supervised Learning in Simulation

Limited power and computational resources, absence of high-end sensor equipment and GPS-denied environments are challenges faced by autonomous micro areal vehicles (MAVs). We address these challenges in the context of autonomous navigation and landing of MAVs in indoor environments and propose a vision-based control approach using Supervised Learning. To achieve this, we collected data samples in a simulation environment which were labelled according to the optimal control command determined by a path planning algorithm. Based on these data samples, we trained a Convolutional Neural Network (CNN) that maps low resolution image and sensor input to high-level control commands. We have observed promising results in both obstructed and non-obstructed simulation environments, showing that our model is capable of successfully navigating a MAV towards a landing platform. Our approach requires shorter training times than similar Reinforcement Learning approaches and can potentially overcome the limitations of manual data collection faced by comparable Supervised Learning approaches.

==> bibliography.tex <==
@article{Airsim,
  author    = {Shital Shah and
               Debadeepta Dey and
               Chris Lovett and
               Ashish Kapoor},
  title     = {AirSim: High-Fidelity Visual and Physical Simulation for Autonomous
               Vehicles},
  journal   = {CoRR},
  volume    = {abs/1705.05065},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.05065},
  archivePrefix = {arXiv},
  eprint    = {1705.05065},
  timestamp = {Mon, 13 Aug 2018 16:46:28 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/ShahDLK17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
